From Paper Trails to Trust on Tracks: Adding Public Transparency to Railways via zk-SNARKs

Railways provide a critical service and operate under strict regulatory frameworks for implementing changes or upgrades. Despite their impact on the public, these frameworks do not define means or mechanisms for transparency towards the public, leading to reduced trust and complex tracking processes. We analyse the German guideline for railway-infrastructural modifications from proposal to approval, using the guideline as a motivating example for modelling decisions in processes using digital signatures and zero-knowledge proofs. Therein, a verifier can verify that a process was executed correctly by the involved parties and according to specification without learning confidential information such as trade secrets or identities of the participants. We validate our system by applying it to the railway process, demonstrating how it realises various rules, and we evaluate its scalability with increased process complexities. Our solution is not railway-specific but also applicable to other contexts, helping leverage zero-knowledge proofs for public transparency and trust.

==> content/solution/business.tex <==
\subsection{Business Rules}

The algorithms from Section~\ref{section:system} enable producing verifiable
evidence that every connection between two nodes satisfies the cryptographic
requirements, it does not tell whether the connection also meets any potential
business requirements.
%
For example, while the cryptographic verification would ensure that node A
delegates node B, business rules determine whether node A can delegate node B
in the first place or not.
%
As the business requirements vary according to process requirements,
organizational policies, or general regulations, we enable two additional
layers of functional verification by specifying a Chain Policy $\chainpolicy$
and a Phase Policy $\phasepolicy$.

\subsubsection{Chain Policy}

Subset-role Delegation as Chain Policy

\subsubsection{Phase Policy}

Some examples for rules that can be imlemented:

\begin{itemize}
    \item Threshold Actions
    \item Reference single
    \item Reference multiple
\end{itemize}


==> content/solution/construction/attestdoc.tex <==
\procedure
[]
{
$\attestdoc(\attestdocinput)$
}
{
    \sig \gets \sigsign(\sk, \docinfo) \\
    \return \docsig := \sigsig
}


==> content/solution/construction/attestrole.tex <==
\procedure
[]
{
$\attestrole(\attestroleinput)$
}
{
    \sig \gets \sigsign(\sk, \pk \| \roleinfo) \\
    \return \rolesig := \sigsig
}


==> content/solution/construction/keygen.tex <==
\procedure
[]
{
$\keygen(\keygeninput)$
}
{
    (\sigkeypair) \gets \sigkeygen(\keygeninput) \\
    \return (\sigkeypair)
}



==> content/solution/construction/verifychain.tex <==
\procedure
[]
{
$\verifychain(\verifychaininput)$
}
{
    \returnif{
       1 
    }
    {
        \sigverify(\pk_0, \docinfo, \docsig) = 1 \ \land \\
        \t[2]
        \forall i \in [n] \ 
        \sigverify(\pk_i, \pk_{i-1} \| \roleinfo_{i-1},\rolesig_i) = 1
         \\
    }
    {
        0
    }
}

